A Framework for Consistency Algorithms

We present a framework that provides deterministic consistency algorithms for given memory models. Such an algorithm checks whether the executions of a shared-memory concurrent program are consistent under the axioms defined by a model. For memory models like SC and TSO, checking consistency is NP-complete. Our framework shows, that despite the hardness, fast deterministic consistency algorithms can be obtained by employing tools from fine-grained complexity. The framework is based on a universal consistency problem which can be instantiated by different memory models. We construct an algorithm for the problem running in time O*(2^k), where k is the number of write accesses in the execution that is checked for consistency. Each instance of the framework then admits an O*(2^k)-time consistency algorithm. By applying the framework, we obtain corresponding consistency algorithms for SC, TSO, PSO, and RMO. Moreover, we show that the obtained algorithms for SC, TSO, and PSO are optimal in the fine-grained sense: there is no consistency algorithm for these running in time 2^o(k) unless the exponential time hypothesis fails.

==> content/unused.tex <==
\begin{comment}
\subparagraph*{ The graph $\graph{mm}(\twWR)$ is acyclic:} 
Towards proving acyclicity of $\graph{mm}(\twWR)$, we will show that the vertices of the graph (i.e. the events in $h_{\formula}$) can be linearised in such a way that the edges of it are forward looking (i.e. from lower position to an higher one in the linear ordering). This will give us a topological sort of the graph, automatically proving that the graph is acyclic. We produce such a linear ordering $\sigma$ inductively. During this inductive construction, we maintain the invariant that in any edge between the vertices of the linear order produced, the forward looking property holds. Before we prove acyclicity of $\graph{mm}(\twWR)$, we make the following simple observations.
\begin{observation} \label{apx:obs:forward}
Let $o \subseteq O(h_{\formula})$ be any subset of events of $h_{\formula}$ and $\gamma = \Linear(o)$ be any linearisation of it. 

\begin{enumerate}
\item  For any $o_1,o_2 \in o$ such that  $(o_1,o_2) \in \rf$, $(o_1,o_2)$ is forward looking in $\gamma$ if and only if $o_1 < o_2$ in $\gamma$.
\item   For any $o_1,o_2,o_3 \in o$ such that $(o_1,o_2) \in \rf$ and $(o_2,o_3) \in \cf$, $(o_2,o_3)$ is forward looking in $\gamma$ if and only   if $o_1 < o_2 < o_3$ in $\gamma$.
\end{enumerate}
\end{observation} 

We now construct a linear ordering $\sigma$ of the events $O(h_{\formula})$, by inducting on the length of the total order. We will use $\Linear(\First(X))$ to mean the linearisation of the threads in $\First(X)$ according to the assumed ordering on the variables. Similarly we use $\Linear(\First(C_{i}))$ for some linearisation of the threads in $ \First(C_{i})$, respecting the ordering of the literals and the program order. We also extend the definition to $\Linear(\Second(X)),  \Linear(\Second(C_{i}))$ Unless specified otherwise, all the events of  a thread appear together in the linearisation.

\begin{itemize}
\item Consider $\sigma_1 = \Linear(\First(X))$, the events in these threads are only the write events, hence we let the linearisation similar to $LWF(X)$.  There are no $\po$ edges between the vertices. Further there are no $\rf$ and $\cf$ edges between them since there are not any reads. Finally since the linearisation of these events is the same as in $\twWR$, hence $\tw$ edges are forward looking. %Hence  the required property is maintained.

\item We now show how to inductively extend $\sigma_1$ with the events that occur in the processes  $\lTransfer0(\ell),\lTransfer1(\ell) $. 
After rounds $i$, assume that the linearisation obtained be $\sigma_1 \cdot \sigma^1_2 \cdot \sigma^2_2 \cdots \sigma^i_2$. We now add the set of events from $\Linear(\First(C_{i+1}))$.  In this case, we not only have writes but also reads. Each of these reads get its values from   $\sigma_1$. Clearly $\tw$ edges are forward looking since the writes happens exactly as in the given total order. Further any value read is already written in $\sigma_1$ hence we have the $\rf$ edges are forward looking. Since the writes so far are still to unique variables, there are no $\cf$ edge.  

\item  We now show how to inductively extend $\sigma_1 \cdot \sigma_2$ with the events that occur in the processes $\ClChecker{*}(C)$ inductively. The events of these threads do not occur contiguously. After $i$ rounds, we assume the linearisation obtained is $\sigma_1 \cdot \sigma_2 \cdot \sigma^1_3 \cdots \sigma^i_3$, we extend this with the events of $O(\ClChecker*(C_{i+1})) = O(\ClChecker1(C_{i+1})) \cup O(\ClChecker2(C_{i+1})) \cup O(\ClChecker3(C_{i+1}))$. Let $\goodSeq(C_{i+1}) = \{ \rd(\ell^{i+1}_j,0) \mid \ell^{i+1}_j  \in \trueClause{i+1}{\true}  \} \cup \{\rd(\ell^{i+1}_j,1) \mid \exists \ell^{i+1}_{j'}  \in \trueClause{i+1}{\true}: \ell^{i+1}_j = \ell^{i+1}_{\Nxt(j')}  \}$. Clearly each of the events in $\goodSeq$ is an event in $O(\ClChecker*(C_{i+1}))$ such that value read by it is  written in $\sigma_2$. Further each of the  events in $\goodSeq$ can be executed since we have only selected those events which are not blocked. We extend the linearisation sequence by adding the elements in the $\goodSeq$, respecting the program order. Clearly any $\rf$ edge is forward looking since the reads come after the writes. n

\item We now show how to extend $\sigma_1 \cdot \sigma_2 \cdot \sigma_3$ with  the events that occur in $\Second(X)$. Since the elements in it are only write events that are not related by $\po$ order, we simply append $\Linear(\Second(X))$. Here we only need to argue about the $\cf,\tw$ edges. For $\tw$ edges, notice that the writes are in same order as in the total order. Since all the reads to the previous write to the same variable occurs before, all the $\cf$ edges are forward looking (see Observation \ref{apx:obs:forward}). As a consequence, we get the sequence $\sigma_1 \cdots \sigma_4$

\item We now show how to extend $\sigma_1 \cdot \sigma_2 \cdot \sigma_3 \cdot \sigma_4$ with  theremaining events that occur in $\lTransfer0(\ell),\lTransfer1(\ell)$, inductively. After rounds $i$, assume that the linearisation obtained be $\sigma_1 \cdots \sigma_4 \cdot \sigma^1_5 \cdot \sigma^2_5 \cdots \sigma^i_5$. We now distinguish between whether the clause $C_{i+1}$ is satisfied by more than one literal or by one literal. If it is by more then one literal, we simply append the events of $\Linear(\Second(C_{i+1}))$. We need to argue that the $\cf$ edges are forward looking. But this is immediate from Observation \ref{apx:obs:forward} since we are adding the writes after the reads in $\sigma_4$.

Suppose $C_{i+1}$ is satisfied by exactly one literal. Then we will have four read events  of $O(\ClChecker{*}(C_{i+1}))$ pending. Of this, one of the read corresponds to the value written in  $\First(C_{i+1})$. Let the literral corresponding to it be $\ell^{i+1}_j$. It is easy to see that a reads is blocked by a read to $\ell^{i+1}_{j'}$ that reads a $0$ from $\Linear(\Second(C_{i+1}))$. By definition,  this literal $\ell^{i+1}_{j'}$ is before $\ell^{i+1}_{j}$ in the literal ordering.  We insert the $\wri(\ell^{i+1}_{j'},0) \cdot \rd(\ell^{i+1}_{j'},0)$ followed by $\rd(\ell^{i+1}_{j},1)$. We then append the rest of $\Linear(\Second(C_{i+1}))$. One can easily check that such a linearisation maintains the required property. The $\cf$ edges are forward looking since the reads are from immediate writes. For the same reason, the $\rf$ edges are forward looking.

\item Finally the remaining reads of the $O(\ClChecker{*})$ are inserted. Clearly the $\rf$ relations are forward looking. Since these are the last reads reading immediate values and there are no further write,  there are no $\cf$ edges starting from these reads.
\end{itemize}
\end{comment}
